Shor's algorithm on a nearest-neighbor machine

We give a new ``nested adds'' circuit for implementing Shor's algorithm in linear width and quadratic depth on a nearest-neighbor machine. Our circuit combines Draper's transform adder with approximation ideas of Zalka. The transform adder requires small controlled rotations. We also give another version, with slightly larger depth, using only reversible classical gates. We do not know which version will ultimately be cheaper to implement.

==> abs.tex <==
\htmlonly{\FOUO}
We give a new ``nested adds'' circuit for implementing Shor's
algorithm in linear width and quadratic depth on a nearest-neighbor
machine.  Our circuit combines Draper's transform adder with
approximation ideas of Zalka.  The transform adder requires small
controlled rotations.  We also give another version, with slightly
larger depth, using only reversible classical gates.  We do not know
which version will ultimately be cheaper to implement.


